A data-based image representation for continuous-time LTI systems

We derive a numerically stable method to compute an image representation of an unknown linear system only from data, leveraging a continuous-time version of Willems et al.'s fundamental lemma. To this end, we use derivatives approximated by algebraic differentiators. Our novel image representation avoids solving differential-algebraic equations and significantly reduces computational complexity by eliminating redundant degrees of freedom corresponding to the number of unknown quantities to be identified. Simulation results confirm the effectiveness of the proposed approach, even in the presence of severe measurement disturbances.

==> figs/20251122_174404/lambda_1p00em08/noise_1p0000e-02/seed_1284858263/paper_plots.tex <==
%\documentclass[border=5pt]{standalone}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.18}
%\usepgfplotslibrary{groupplots}
%
%\begin{document}

	\begin{tikzpicture}
		\begin{groupplot}[
			group style={
				group size=1 by 1,
				vertical sep=0.45cm,
				xlabels at=edge bottom,
			},
			width=8.8cm,
			height=3cm,
			grid=major,
			xmin=0,
			xmax = 16,
			]
			
			
			% Subplot 3: State trajectory
			\nextgroupplot[ylabel=signals, xlabel=$t$,	legend style={at={(0.5,1.5)}, anchor=north, legend columns=4, draw=none},]
			\addplot[line width=0.75pt, blue] table[x index=0, y index=1] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_1$}
			\addplot[line width=0.75pt, green] table[x index=0, y index=2] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_2$}
			\addplot[line width=0.75pt, orange] table[x index=0, y index=3] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_3$}
			
			
			\addplot[xlabel={$t$},line width=0.75pt, black, dash pattern={on 10pt off 2pt on 1pt off 3pt},] table[x index=0, y index=4] {traj_state_down.dat};
			\addlegendentry{${x}_i$}
			\addplot[line width=0.75pt, black, dash pattern={on 10pt off 2pt on 1pt off 3pt},] table[x index=0, y index=5] {traj_state_down.dat};
			\addplot[line width=0.75pt, black, dash pattern={on 10pt off 2pt on 1pt off 3pt},] table[x index=0, y index=6] {traj_state_down.dat};
			% Subplot 2: Output trajectory
%			\nextgroupplot[ylabel=input,			legend style={at={(0.7,0.3)}, anchor=north, legend columns=2, draw=none},]
%			\addplot[line width=0.75pt, blue] table[x index=0, y index=1] {traj_input_down.dat};
%%			\addlegendentry{$u$}
			
		\end{groupplot}
	\end{tikzpicture}
%\end{document}


==> figs/20251122_174404/lambda_1p00em08/noise_1p0000e-02/seed_1284858263/paper_plots_training_Data.tex <==
\begin{tikzpicture}
	% Left axis: outputs (y and \tilde{y})
	\begin{axis}[
		name=leftaxis,
		width=7.8cm,
		height=2.8cm,
		grid=major,
		xmin=0,
		xmax = 8,
		xlabel={$t$},
		ylabel={output},
		axis x line*=bottom,
		axis y line*=left,
		legend style={at={(0.183,0.99)}, anchor=north, legend columns=2, fill=white, draw=none},
		]
		% noisy output \tilde{y}
		\addplot[line width=0.75pt, red, opacity=0.6]
		table[x index=0, y index=1] {pe_output.dat};
		% \addlegendentry{$\bar{y}_\eta$}
		
		% true output y
		\addplot[black, dash pattern={on 10pt off 2pt on 1pt off 3pt}, line width=0.75pt]
		table[x index=0, y index=2] {pe_output.dat};
		% \addlegendentry{$\bar y$}
	\end{axis}
	
	% Right axis: input u_PE (overlaid)
	\begin{axis}[
		width=7.8cm,
		height=2.8cm,
		at={(leftaxis.south east)},
		anchor=south east,
%		axis x line=none,      % no second x-axis line
		axis y line*=right,
		ylabel={input},
		xmin=0,
		xmax = 8,
%		ymin=0, ymax=0,        % let pgfplots auto-scale; remove or adjust as needed
		yticklabel style={/pgf/number format/fixed},
		legend style={at={(0.45,0.98)}, anchor=north, legend columns=1, fill=white, draw=none},
		]
		\addplot[line width=0.75pt]
		table[x index=0, y index=1] {pe_input.dat};
		% \addlegendentry{$\bar u$}
	\end{axis}
\end{tikzpicture}


==> figs/20251122_174404/lambda_1p00em08/noise_2p0000e-02/seed_1432881518/paper_plots.tex <==
%\documentclass[border=5pt]{standalone}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.18}
%\usepgfplotslibrary{groupplots}
%
%\begin{document}
	\begin{tikzpicture}
		\begin{groupplot}[
			group style={
				group size=1 by 1,
				vertical sep=1.0cm,
				xlabels at=edge bottom,
			},
			width=8cm,
			height=4cm,
			xlabel={$t$},
			grid=major,
			xmin=0,
			xmax = 16,
			]
			
			
			% Subplot 3: State trajectory
			\nextgroupplot[xlabel={$t$},ylabel=signals,	legend style={at={(0.5,1.25)}, anchor=north, legend columns=4, draw=none},]
			\addplot[line width=2pt, blue] table[x index=0, y index=1] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_1$}
			\addplot[line width=2pt, green] table[x index=0, y index=2] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_2$}
			\addplot[line width=2pt, orange] table[x index=0, y index=3] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_3$}
			
			
			\addplot[line width=2pt, black, dashed,] table[x index=0, y index=4] {traj_state_down.dat};
			\addlegendentry{${x}_i$}
			\addplot[line width=2pt, black, dashed,] table[x index=0, y index=5] {traj_state_down.dat};
			\addplot[line width=2pt, black, dashed,] table[x index=0, y index=6] {traj_state_down.dat};
			% Subplot 2: Output trajectory
%			\nextgroupplot[ylabel
%			\addlegendentry{$u$}
			
		\end{groupplot}
	\end{tikzpicture}
%\end{document}


==> figs/20251122_174404/lambda_1p00em08/noise_2p0000e-02/seed_1432881518/paper_plots_training_Data.tex <==
\begin{tikzpicture}
	% Left axis: outputs (y and \tilde{y})
	\begin{axis}[
		name=leftaxis,
		width=7.0cm,
		height=4cm,
		grid=major,
		xmin=0,
		xmax = 8,
		xlabel={$t$},
		ylabel={output},
		axis x line*=bottom,
		axis y line*=left,
		legend style={at={(0.5,1.0)}, anchor=north, legend columns=2, draw=none},
		]
		% noisy output \tilde{y}
		\addplot[line width=2pt, red, opacity=0.6]
		table[x index=0, y index=1] {pe_output.dat};
		\addlegendentry{$\tilde{y}$}
		
		% true output y
		\addplot[black, dashed, line width=2pt]
		table[x index=0, y index=2] {pe_output.dat};
		\addlegendentry{$y$}
	\end{axis}
	
	% Right axis: input u_PE (overlaid)
	\begin{axis}[
		width=7.0cm,
		height=4cm,
		at={(leftaxis.south east)},
		anchor=south east,
%		axis x line=none,      % no second x-axis line
		axis y line*=right,
		ylabel={input},
		xmin=0,
		xmax = 8,
%		ymin=0, ymax=0,        % let pgfplots auto-scale; remove or adjust as needed
		yticklabel style={/pgf/number format/fixed},
		legend style={at={(0.8,1.0)}, anchor=north, legend columns=1, draw=none},
		]
		\addplot[line width=2pt]
		table[x index=0, y index=1] {pe_input.dat};
		\addlegendentry{$u$}
	\end{axis}
\end{tikzpicture}


==> figs/20251122_174404/lambda_1p00em08/noise_2p0000e-02/seed_211875280/paper_plots.tex <==
%\documentclass[border=5pt]{standalone}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.18}
%\usepgfplotslibrary{groupplots}
%
%\begin{document}

	\begin{tikzpicture}
		\begin{groupplot}[
			group style={
				group size=1 by 1,
				vertical sep=0.45cm,
				xlabels at=edge bottom,
			},
			width=8cm,
			height=4cm,
			grid=major,
			xmin=0,
			xmax = 16,
			]
			
			
			% Subplot 3: State trajectory
			\nextgroupplot[ylabel=signals, xlabel=$t$,	legend style={at={(0.5,1.25)}, anchor=north, legend columns=4, draw=none},]
			\addplot[line width=2pt, blue] table[x index=0, y index=1] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_1$}
			\addplot[line width=2pt, green] table[x index=0, y index=2] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_2$}
			\addplot[line width=2pt, orange] table[x index=0, y index=3] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_3$}
			
			
			\addplot[xlabel={$t$},line width=2pt, black, dashed,] table[x index=0, y index=4] {traj_state_down.dat};
			\addlegendentry{${x}_i$}
			\addplot[line width=2pt, black, dashed,] table[x index=0, y index=5] {traj_state_down.dat};
			\addplot[line width=2pt, black, dashed,] table[x index=0, y index=6] {traj_state_down.dat};
			% Subplot 2: Output trajectory
%			\nextgroupplot[ylabel=input,			legend style={at={(0.7,0.3)}, anchor=north, legend columns=2, draw=none},]
%			\addplot[line width=2pt, blue] table[x index=0, y index=1] {traj_input_down.dat};
%%			\addlegendentry{$u$}
			
		\end{groupplot}
	\end{tikzpicture}
%\end{document}


==> figs/20251122_174404/lambda_1p00em08/noise_2p0000e-02/seed_211875280/paper_plots_training_Data.tex <==
\begin{tikzpicture}
	% Left axis: outputs (y and \tilde{y})
	\begin{axis}[
		name=leftaxis,
		width=7.0cm,
		height=4cm,
		grid=major,
		xmin=0,
		xmax = 8,
		xlabel={$t$},
		ylabel={output},
		axis x line*=bottom,
		axis y line*=left,
		legend style={at={(0.3,0.98)}, anchor=north, legend columns=2, draw=none},
		]
		% noisy output \tilde{y}
		\addplot[line width=1pt, red, opacity=0.6]
		table[x index=0, y index=1] {pe_output.dat};
		\addlegendentry{$\tilde{y}$}
		
		% true output y
		\addplot[black, dashed, line width=2pt]
		table[x index=0, y index=2] {pe_output.dat};
		\addlegendentry{$y$}
	\end{axis}
	
	% Right axis: input u_PE (overlaid)
	\begin{axis}[
		width=7.0cm,
		height=4cm,
		at={(leftaxis.south east)},
		anchor=south east,
%		axis x line=none,      % no second x-axis line
		axis y line*=right,
		ylabel={input},
		xmin=0,
		xmax = 8,
%		ymin=0, ymax=0,        % let pgfplots auto-scale; remove or adjust as needed
		yticklabel style={/pgf/number format/fixed},
		legend style={at={(0.6,0.98)}, anchor=north, legend columns=1, draw=none},
		]
		\addplot[line width=2pt]
		table[x index=0, y index=1] {pe_input.dat};
		\addlegendentry{$u$}
	\end{axis}
\end{tikzpicture}


==> figs/20251122_174404/lambda_1p00em08/noise_2p0000e-02/seed_384319804/paper_plots.tex <==
%\documentclass[border=5pt]{standalone}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.18}
%\usepgfplotslibrary{groupplots}
%
%\begin{document}

	\begin{tikzpicture}
		\begin{groupplot}[
			group style={
				group size=1 by 1,
				vertical sep=0.45cm,
				xlabels at=edge bottom,
			},
			width=8cm,
			height=4cm,
			grid=major,
			xmin=0,
			xmax = 16,
			]
			
			
			% Subplot 3: State trajectory
			\nextgroupplot[ylabel=signals, xlabel=$t$,	legend style={at={(0.5,1.25)}, anchor=north, legend columns=4, draw=none},]
			\addplot[line width=2pt, blue] table[x index=0, y index=1] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_1$}
			\addplot[line width=2pt, green] table[x index=0, y index=2] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_2$}
			\addplot[line width=2pt, orange] table[x index=0, y index=3] {traj_state_down.dat};
			\addlegendentry{$\hat{x}_3$}
			
			
			\addplot[xlabel={$t$},line width=2pt, black, dashed,] table[x index=0, y index=4] {traj_state_down.dat};
			\addlegendentry{${x}_i$}
			\addplot[line width=2pt, black, dashed,] table[x index=0, y index=5] {traj_state_down.dat};
			\addplot[line width=2pt, black, dashed,] table[x index=0, y index=6] {traj_state_down.dat};
			% Subplot 2: Output trajectory
%			\nextgroupplot[ylabel=input,			legend style={at={(0.7,0.3)}, anchor=north, legend columns=2, draw=none},]
%			\addplot[line width=2pt, blue] table[x index=0, y index=1] {traj_input_down.dat};
%%			\addlegendentry{$u$}
			
		\end{groupplot}
	\end{tikzpicture}
%\end{document}


==> figs/20251122_174404/lambda_1p00em08/noise_2p0000e-02/seed_384319804/paper_plots_training_Data.tex <==
\begin{tikzpicture}
	% Left axis: outputs (y and \tilde{y})
	\begin{axis}[
		name=leftaxis,
		width=7.0cm,
		height=4cm,
		grid=major,
		xmin=0,
		xmax = 8,
		xlabel={$t$},
		ylabel={output},
		axis x line*=bottom,
		axis y line*=left,
		legend style={at={(0.3,0.98)}, anchor=north, legend columns=2, draw=none},
		]
		% noisy output \tilde{y}
		\addplot[line width=1pt, red, opacity=0.6]
		table[x index=0, y index=1] {pe_output.dat};
		\addlegendentry{$\tilde{y}$}
		
		% true output y
		\addplot[black, dashed, line width=2pt]
		table[x index=0, y index=2] {pe_output.dat};
		\addlegendentry{$y$}
	\end{axis}
	
	% Right axis: input u_PE (overlaid)
	\begin{axis}[
		width=7.0cm,
		height=4cm,
		at={(leftaxis.south east)},
		anchor=south east,
%		axis x line=none,      % no second x-axis line
		axis y line*=right,
		ylabel={input},
		xmin=0,
		xmax = 8,
%		ymin=0, ymax=0,        % let pgfplots auto-scale; remove or adjust as needed
		yticklabel style={/pgf/number format/fixed},
		legend style={at={(0.6,0.98)}, anchor=north, legend columns=1, draw=none},
		]
		\addplot[line width=2pt]
		table[x index=0, y index=1] {pe_input.dat};
		\addlegendentry{$u$}
	\end{axis}
\end{tikzpicture}

